Textoshop: Interactions Inspired by Drawing Software to Facilitate Text Editing

We explore how interactions inspired by drawing software can help edit text. Making an analogy between visual and text editing, we consider words as pixels, sentences as regions, and tones as colours. For instance, direct manipulations move, shorten, expand, and reorder text; tools change number, tense, and grammar; colours map to tones explored along three dimensions in a tone picker; and layers help organize and version text. This analogy also leads to new workflows, such as boolean operations on text fragments to construct more elaborated text. A study shows participants were more successful at editing text and preferred using the proposed interface over existing solutions. Broadly, our work highlights the potential of interaction analogies to rethink existing workflows, while capitalizing on familiar features.

==> _setup.tex <==
% Exii Standard Document Setup
% ================================

% various standard exii macros
\usepackage{exii-macros}

% additional latex packages
\usepackage{booktabs}

% Author comments
% See exii-macros.sty for colours the last line and choose a colour
% IMPORTANT: also enter texcount TC macros for each author!
% (otherwise even hidden comments are included in the word count)

% also ignore outline comments
%TC:macro \outline [ignore]

% macros specific to this project
\newcommand{\name}{Textoshop\xspace}

% Annotation Visibility Control
% --------------------------------

% *** HIDE INLINE COMMENTS HERE ***
% command below will hide all author comments, simple comments like guide, and 
% make markup comments like fixme return to black text
% \hidecomments
% or, just hide the grey outline comments
% \hideoutline

% *** CAMERA-READY REVISION HIGHLIGHTING ***
% command below highlights major revisions when submitting camera-ready. In text, you need to wrap major revisions sections with \rev macro.
%\showrevisions{REVISIONGREEN}

% Formatting Tweaks
% --------------------------------

% *** NICE DRAFT FORMAT WITH HANDWRITTEN MARK-UP SPACE (ACM ONLY) ***
% Increase margins and line spacing to make it easier 
% to markup a 1-column PDF with handwritten comments. 
% Use this with format=acmsmall in documentclass
% Note this causes a latex error because the acmart template
% doesn't allow you to change baselinestretch (but we only
% change it for our internal drafts using this command}
% \addmarkupspace

% By default, the template aligns the columns at the bottom of each page.
% This inserts uneven vertical spacing between paragraphs with looks awful, 
% and wastes space. Using a "ragged bottom" is better.
%\raggedbottom

% The template has insanely huge space around captions, we can reduce this.
% Be cautious, some white space is needed to separate caption from text. 
%\setlength{\abovecaptionskip}{3pt}
%\setlength{\belowcaptionskip}{-3pt}



% cheat by reducing line spacing: AVOID DOING THIS UNLESS DESPERATE!
% \renewcommand{\baselinestretch}{0.95} % default is 1.0
